The bright-end galaxy candidates at z ~ 9 from 79 independent HST fields

We present a full data analysis of the pure-parallel Hubble Space Telescope (HST) imaging observations in the Brightest of Reionizing Galaxies Survey (BoRG[z9]) in Cycle 22. The medium-deep exposures with five HST/WFC3IR+UVIS filter bands from 79 independent sightlines (~370 arcmin^2) provide the least biased determination of number density for z>9 bright galaxies against cosmic variance. After a strict two-step selection for candidate galaxies, including dropout color and photometric redshift analyses, and revision of previous BoRG candidates, we identify one source at z~10 and two sources at z~9. The z~10 candidate shows evidence of line-of-sight lens magnification (mu~1.5), yet it appears surprisingly luminous (MUV ~ -22.6\pm0.3 mag), making it one of the brightest candidates at z > 8 known (~ 0.3 mag brighter than the z = 8.68 galaxy EGSY8p7, spectroscopically confirmed by Zitrin and collaborators). For z ~ 9 candidates, we include previous data points at fainter magnitudes and find that the data are well fitted by a Schechter luminosity function with alpha ~ -2.1, MUV ~ -21.5 mag, and log phi ~ -4.5 Mpc^-3mag^-1, for the first time without fixing any parameters. The inferred cosmic star formation rate density is consistent with unaccelerated evolution from lower redshift.

==> fig_cand.tex <==
\includegraphics[width=0.60\textwidth]{Fig/JH_2140+0241_303.pdf}
\includegraphics[width=0.39\textwidth]{Fig/prior_sim_borg_jh_2140+0241-303_spitz.pdf}
\includegraphics[width=0.60\textwidth]{Fig/YJH_0751+2917_499.pdf}
\includegraphics[width=0.39\textwidth]{Fig/prior_sim_borg_yjh_0751+2917-499.pdf}
\includegraphics[width=0.60\textwidth]{Fig/YJH_0807+3606_774.pdf}
\includegraphics[width=0.39\textwidth]{Fig/prior_sim_borg_yjh_0807+3606-774.pdf}
\includegraphics[width=0.60\textwidth]{Fig/YJH_0956+2848_98.pdf}
\includegraphics[width=0.39\textwidth]{Fig/prior_sim_borg_yjh_0956+2848-98.pdf}
\includegraphics[width=0.60\textwidth]{Fig/YJH_2229-0945_394.pdf}
\includegraphics[width=0.39\textwidth]{Fig/prior_sim_borg_yjh_2229-0945-394.pdf}


==> fig_cand_yjh_rej.tex <==
\includegraphics[width=0.60\textwidth]{Fig/YJH_0116+1425_442.pdf}
\includegraphics[width=0.39\textwidth]{Fig/prior_sim_borg_yjh_0116+1425-442.pdf}
\includegraphics[width=0.60\textwidth]{Fig/YJH_0119-3411_516.pdf}
\includegraphics[width=0.39\textwidth]{Fig/prior_sim_borg_yjh_0119-3411-516.pdf}
\includegraphics[width=0.60\textwidth]{Fig/YJH_0314-6712_1393.pdf}
\includegraphics[width=0.39\textwidth]{Fig/prior_sim_borg_yjh_0314-6712-1393.pdf}
\includegraphics[width=0.60\textwidth]{Fig/YJH_0337-0507_775.pdf}
\includegraphics[width=0.39\textwidth]{Fig/prior_sim_borg_yjh_0337-0507-775.pdf}
\includegraphics[width=0.60\textwidth]{Fig/YJH_0554-6005_812.pdf}
\includegraphics[width=0.39\textwidth]{Fig/prior_sim_borg_yjh_0554-6005-812.pdf}
\includegraphics[width=0.60\textwidth]{Fig/YJH_0554-6005_890.pdf}
\includegraphics[width=0.39\textwidth]{Fig/prior_sim_borg_yjh_0554-6005-890.pdf}
\includegraphics[width=0.60\textwidth]{Fig/YJH_0751+2917_410.pdf}
\includegraphics[width=0.39\textwidth]{Fig/prior_sim_borg_yjh_0751+2917-410.pdf}
\includegraphics[width=0.60\textwidth]{Fig/YJH_0807+3606_157.pdf}
\includegraphics[width=0.39\textwidth]{Fig/prior_sim_borg_yjh_0807+3606-157.pdf}
\includegraphics[width=0.60\textwidth]{Fig/YJH_0952+5150_162.pdf}
\includegraphics[width=0.39\textwidth]{Fig/prior_sim_borg_yjh_0952+5150-162.pdf}
\includegraphics[width=0.60\textwidth]{Fig/YJH_1015+5945_850.pdf}
\includegraphics[width=0.39\textwidth]{Fig/prior_sim_borg_yjh_1015+5945-850.pdf}
\includegraphics[width=0.60\textwidth]{Fig/YJH_1017-2052_119.pdf}
\includegraphics[width=0.39\textwidth]{Fig/prior_sim_borg_yjh_1017-2052-119.pdf}
\includegraphics[width=0.60\textwidth]{Fig/YJH_1104+2813_156.pdf}
\includegraphics[width=0.39\textwidth]{Fig/prior_sim_borg_yjh_1104+2813-156.pdf}
\includegraphics[width=0.60\textwidth]{Fig/YJH_1142+2647_134.pdf}
\includegraphics[width=0.39\textwidth]{Fig/prior_sim_borg_yjh_1142+2647-134.pdf}
\includegraphics[width=0.60\textwidth]{Fig/YJH_1152+3402_152.pdf}
\includegraphics[width=0.39\textwidth]{Fig/prior_sim_borg_yjh_1152+3402-152.pdf}
\includegraphics[width=0.60\textwidth]{Fig/YJH_1152+3402_186.pdf}
\includegraphics[width=0.39\textwidth]{Fig/prior_sim_borg_yjh_1152+3402-186.pdf}
\includegraphics[width=0.60\textwidth]{Fig/YJH_1152+5433_577.pdf}
\includegraphics[width=0.39\textwidth]{Fig/prior_sim_borg_yjh_1152+5433-577.pdf}
\includegraphics[width=0.60\textwidth]{Fig/YJH_1152+5433_664.pdf}
\includegraphics[width=0.39\textwidth]{Fig/prior_sim_borg_yjh_1152+5433-664.pdf}
\includegraphics[width=0.60\textwidth]{Fig/YJH_1152+5434_790.pdf}
\includegraphics[width=0.39\textwidth]{Fig/prior_sim_borg_yjh_1152+5434-790.pdf}
\includegraphics[width=0.60\textwidth]{Fig/YJH_1209+4543_784.pdf}
\includegraphics[width=0.39\textwidth]{Fig/prior_sim_borg_yjh_1209+4543-784.pdf}
\includegraphics[width=0.60\textwidth]{Fig/YJH_1438-0142_939.pdf}
\includegraphics[width=0.39\textwidth]{Fig/prior_sim_borg_yjh_1438-0142-939.pdf}
\includegraphics[width=0.60\textwidth]{Fig/YJH_1442-0212_600.pdf}
\includegraphics[width=0.39\textwidth]{Fig/prior_sim_borg_yjh_1442-0212-600.pdf}
\includegraphics[width=0.60\textwidth]{Fig/YJH_1519-0746_179.pdf}
\includegraphics[width=0.39\textwidth]{Fig/prior_sim_borg_yjh_1519-0746-179.pdf}
\includegraphics[width=0.60\textwidth]{Fig/YJH_1520-2501_228.pdf}
\includegraphics[width=0.39\textwidth]{Fig/prior_sim_borg_yjh_1520-2501-228.pdf}
\includegraphics[width=0.60\textwidth]{Fig/YJH_1525+0960_205.pdf}
\includegraphics[width=0.39\textwidth]{Fig/prior_sim_borg_yjh_1525+0960-205.pdf}
\includegraphics[width=0.60\textwidth]{Fig/YJH_1525+0960_568.pdf}
\includegraphics[width=0.39\textwidth]{Fig/prior_sim_borg_yjh_1525+0960-568.pdf}
\includegraphics[width=0.60\textwidth]{Fig/YJH_1558+0812_897.pdf}
\includegraphics[width=0.39\textwidth]{Fig/prior_sim_borg_yjh_1558+0812-897.pdf}
\includegraphics[width=0.60\textwidth]{Fig/YJH_1920-4531_152.pdf}
\includegraphics[width=0.39\textwidth]{Fig/prior_sim_borg_yjh_1920-4531-152.pdf}
\includegraphics[width=0.60\textwidth]{Fig/YJH_1920-4531_375.pdf}
\includegraphics[width=0.39\textwidth]{Fig/prior_sim_borg_yjh_1920-4531-375.pdf}
\includegraphics[width=0.60\textwidth]{Fig/YJH_1920-4531_515.pdf}
\includegraphics[width=0.39\textwidth]{Fig/prior_sim_borg_yjh_1920-4531-515.pdf}
\includegraphics[width=0.60\textwidth]{Fig/YJH_1920-4531_934.pdf}
\includegraphics[width=0.39\textwidth]{Fig/prior_sim_borg_yjh_1920-4531-934.pdf}
\includegraphics[width=0.60\textwidth]{Fig/YJH_2008-6610_77.pdf}
\includegraphics[width=0.39\textwidth]{Fig/prior_sim_borg_yjh_2008-6610-77.pdf}
\includegraphics[width=0.60\textwidth]{Fig/YJH_2229-0945_755.pdf}
\includegraphics[width=0.39\textwidth]{Fig/prior_sim_borg_yjh_2229-0945-755.pdf}
\includegraphics[width=0.60\textwidth]{Fig/YJH_2312-1423_713.pdf}
\includegraphics[width=0.39\textwidth]{Fig/prior_sim_borg_yjh_2312-1423-713.pdf}
\includegraphics[width=0.60\textwidth]{Fig/YJH_2312-1423_763.pdf}
\includegraphics[width=0.39\textwidth]{Fig/prior_sim_borg_yjh_2312-1423-763.pdf}

